LLM-Enhanced Multiple Instance Learning for Joint Rumor and Stance Detection with Social Context Information

The proliferation of misinformation, such as rumors on social media, has drawn significant attention, prompting various expressions of stance among users. Although rumor detection and stance detection are distinct tasks, they can complement each other. Rumors can be identified by cross-referencing stances in related posts, and stances are influenced by the nature of the rumor. However, existing stance detection methods often require post-level stance annotations, which are costly to obtain. We propose a novel LLM-enhanced MIL approach to jointly predict post stance and claim class labels, supervised solely by claim labels, using an undirected microblog propagation model. Our weakly supervised approach relies only on bag-level labels of claim veracity, aligning with multi-instance learning (MIL) principles. To achieve this, we transform the multi-class problem into multiple MIL-based binary classification problems. We then employ a discriminative attention layer to aggregate the outputs from these classifiers into finer-grained classes. Experiments conducted on three rumor datasets and two stance datasets demonstrate the effectiveness of our approach, highlighting strong connections between rumor veracity and expressed stances in responding posts. Our method shows promising performance in joint rumor and stance detection compared to the state-of-the-art methods.

==> backup.tex <==
\textbf{Token-level Transformer.}\label{sec:TokenTrans}
The core idea of token-level transformer is to model the interactions between words at different positions to jointly attend to tokens from different representation spaces. We perform token-level transformer because it would be more reasonable to make the model learn the importance of the word vectors in sentence representation~\cite{huang2021mixed}. We represent each post as a word sequence $t_i=(w_{i,1}, w_{i,2}, \cdots, w_{i,n})$, where $w_{i,j}$ is a $d$-dimensional vector that can be initialized with pre-trained word embeddings. We then map each word embedding into a fixed-size hidden vector by passing the sequence of word tokens through 6 number of Multi-Head Self-Attention (MHSA) layers, which is derived from default settings in Transformer encoder~\cite{vaswani2017attention}. In detail, MHSA layers transform the input sequence into multiple subspaces with different linear projections:
\begin{equation}\label{equ:Token-levelAtt}
\begin{split}
    & Q_i^h, K_i^h, V_i^h = t_i \cdot W_Q^h, t_i \cdot W_K^h, t_i \cdot W_V^h \\
    & \tilde{t}_i^h = softmax(\frac{Q_i^h \cdot {K_i^h}^T}{\sqrt{d_h}})\cdot V_i^h
\end{split}
\end{equation}
where $Q_i^h, K_i^h, V_i^h$ are the query, key, and value embeddings, respectively, $W_Q^h, W_K^h, W_V^h$ represent parameters related to the $h-th$ head, $\tilde{t}_i^h$ denotes the output states, $\sqrt{d_h}$ is the scaling factor and $d_h$ represents the dimensionality of the $h-th$ head. After that we concatenate all the heads outputs as $\tilde{t}_i = [\tilde{t}_i^1, \tilde{t}_i^2, \cdots, \tilde{t}_i^{n_{t-level}}] \in \mathbb{R}^{|t_i|*d}$, and then feed the concatenation embedding into a normalization layer (layerNorm), and a feed-forward network (FFN), which is consistent with Transformer encoder settings~\cite{vaswani2017attention}.
\begin{equation}\label{equ:layerNorm&FFN}
    \begin{split}
        & L_i = layerNorm(\tilde{t}_i \cdot W_L + \tilde{t}_i)\\
        & F_i = FFN(L_i \cdot W_F + L_i)
    \end{split}
\end{equation}
where $F_i=[s_1; \cdots; s_{|t_i|}] \in \mathbb{R}^{{|t_i|}*d}$ is the matrix representing all words vectors in tweet $t_i$, as such, this transforms $t_i=(w_{i,1} w_{i,2} \cdots w_{i,|t_i|})$ to $F_i=[s_1; \cdots; s_{|t_i|}]$. After which, we get the sentence representation for each tweet by placing the attention mechanism to interpolate all the word vectors:
\begin{equation}\label{equ:Token-leveFinalAtt}
    \begin{split}
        & \alpha_i= softmax(\gamma^T s_i) \\
        & h_i=\sum_{k=0}^{|t_i|} \alpha_i s_i\\
    \end{split}
\end{equation}
where $\gamma \in d, \alpha_k \in \mathbb{R}$, $s_i$ is the word vector obtained in Equation~\ref{equ:layerNorm&FFN}. Claim embedding $h_c$ will also be obtained from the above token-level transformer. And these sentence embeddings for the claim and posts will then be fed into post-level transformer.

\textbf{Post-level Transformer.}\label{sec:PostTrans}
Our goal is to cross-check all the posts in a conversation thread to enhance the post representation, this is because posts in social media are naturally short, and some posts may not have a response or repost, and the stance expressed by each post is highly relevant to other posts in the same conversation thread. We could capture the coherent opinions in a conversation thread by lowering the weight of incorrect information (e.g. a denial posts towards a true claim). To this end, we smoothen the conversation threads by arranging the claim and posts chronologically in a linear structure as shown in Figure~\ref{fig:SequentialModel}, which arranges the source claim as the first post. Then we utilize transformer-based network to make the pairwise comparisons within the conversation thread, to capture users' stances and boost each post's representation. We pass the sentence embeddings: $[h_c, h_1, \cdots, h_n]$, obtained in Sec~\ref{sec:TokenTrans} through $n_{p-level}$ number of MHSA layers to model the information flows in a conversation thread. After passing through these MHSA layers, the output embeddings will also go through layerNorm and FFN as Equation~\ref{equ:layerNorm&FFN} shows. Lastly, we also use an attention mechanism to interpolate the posts before feeding them into downstream architecture, which is consistent with the transformation in Equation~\ref{equ:Token-leveFinalAtt}. As such, this transforms $[h_c, h_1, \cdots, h_n]$ to $[h'_c, h'_1, \cdots, h'_n]$.

